Procedural Synthesis of Remote Sensing Images for Robust Change Detection with Neural Networks

Data-driven methods such as convolutional neural networks (CNNs) are known to deliver state-of-the-art performance on image recognition tasks when the training data are abundant. However, in some instances, such as change detection in remote sensing images, annotated data cannot be obtained in sufficient quantities. In this work, we propose a simple and efficient method for creating realistic targeted synthetic datasets in the remote sensing domain, leveraging the opportunities offered by game development engines. We provide a description of the pipeline for procedural geometry generation and rendering as well as an evaluation of the efficiency of produced datasets in a change detection scenario. Our evaluations demonstrate that our pipeline helps to improve the performance and convergence of deep learning models when the amount of real-world data is severely limited.

==> 01-introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Remote sensing data is utilized in a broad range of industrial applications including emergency mapping, deforestation and wildfire monitoring, detection of illegal construction and urban growth tracking. These data, such as satellite imagery and aerial photographs, can be used, for instance, to recognize land objects and detect changes on the Earth's surface. However, one must deal with the high variability of the remote sensing data (\eg, handle diverse weather conditions, imaging equipment, and regional differences), therefore, it is highly desirable to have automated and highly robust approaches to reduce labour costs.

Recently, data-driven approaches such as deep convolutional neural networks (CNNs) have seen impressive progress on a number of vision tasks, including semantic segmentation, object detection, and change detection~\cite{cheng2017remote,chen2017deeplab,buslaev2018fully,he2017mask,lin2018focal,lin2017feature,alcantarilla2018street}. Such methods offer promising tools for remote sensing applications as they can achieve high performance by leveraging the diversity of the available imagery~\cite{bai2018towards,daudt2018urban,kemker2017deep}. However, in order to successfully operate, most data-driven methods require large amounts of high-quality annotated data~\cite{Gaidon2018,kemker2017deep,gaidon2016virtual,dosovitskiy2017carla}. Obtaining such data in the context of remote sensing poses a significant challenge, as (1)~aerial imagery data are expensive, (2)~collection of raw data with satisfactory coverage and diversity is laborious, costly and error-prone, as is (3)~manual image annotation; (4)~moreover, in some instances such as change detection, the cost of collecting a representative number of rarely occurring cases can be prohibitively high. Unsurprisingly, despite public real-world annotated remote sensing datasets exist~\cite{novikov2018satellite,anniballe2018earthquake,fujita2017damage,daudt2018urban}, these challenges have kept them limited in size, compared to general-purpose vision datasets such as the ImageNet~\cite{deng2009imagenet}. 

Alternatives have been considered to avoid dataset collection issues by producing synthetic annotated images with the aid of game development software such as \emph{Unity}~\cite{unity3d}, \emph{Unreal Engine 4}~\cite{ue4}, and \emph{CRYENGINE}~\cite{cryengine}. This approach has enjoyed adoption in the vision community and has been demonstrated to improve the performance of computer vision algorithms in some instances~\cite{chen2015deepdriving,muller2018sim4cv,Gaidon2018,qiu2016unrealcv,dosovitskiy2017carla,richter2016playing,shah2018airsim}. Its attractive benefits include (1) flexibility in scene composition, reducing the dependency on the occurrence of unbalanced classes, (2) full pixel-level precision without any manual annotation necessary, and (3) the possibility to utilize existing transfer learning techniques for subsequent ``fine-tuning'' on real data. However, little work has been done in the direction of using game engines to produce synthetic datasets in the remote sensing domain, an area that has its own challenges. Executing procedural changes on large-scale urban scenes consisting of many objects is computationally demanding and requires significant optimization either at the scene-level (rendering settings, shaders optimization, shadow casting, etc.) or the object-level (tuning of polygons and textures quality). To achieve sufficient realism, one needs to either spend much time modeling and optimizing the scene or buy ready-made assets, which are expensive and unoptimized. Thus, research on construction of synthetic datasets would contribute to a wider adoption of data-driven methods in the remote sensing domain.

In this work, we explore the emerging possibilities offered by game engines in the context of remote sensing applications. We focus on the challenging task of change detection as our main application, however, it is straightforward to adapt our method to other applications such as semantic segmentation. By leveraging the existing 3D tools, we design and implement an automated pipeline for procedural generation of realistic synthetic data. Our approach uses publicly available cartographic data and produces, on their basis, 3D scenes of real territory (\eg, relief, buildings), which allows us to generate highly realistic 3D models and is necessary in some applications, for instance, when performing an emergency mapping of particular areas during natural disasters. These 3D scenes are rendered using \emph{Unity} engine to produce high-resolution synthetic RGB images. Taking advantage of real cartographic data and simulating a number of image acquisition conditions, we create a large and diverse dataset with a low \emph{simulated-to-real} shift, which allows us to efficiently apply deep learning methods. We validate our data generation pipeline on the change detection task using a state-of-the-art deep CNN. 
We observe consistent improvements in performance and convergence of our models on this task with our synthetic data, compared to when using (scarse) real-world data only. 

In summary, our contributions in this work are:
\begin{itemize}
    \item We describe a semi-automatic pipeline for procedural generation of realistic synthetic images for change detection in the domain of remote sensing.
    
    \item We demonstrate the effectiveness of large volumes of targeted synthetic images for deep learning-based change detection using extensive experiments and a real-world evaluation dataset.
\end{itemize}

The rest of this paper is organized as follows.
In Section~\ref{sec:related}, we review prior work on change detection in the remote sensing domain, including existing image datasets, data generation tools, computational models, and transfer learning techniques. Section~\ref{sec:methods} presents our data generation pipeline. Section~\ref{sec:experiments} poses three experiments investigating the possible benefits of our approach and presents their results. We conclude with a discussion of our results in Section~\ref{sec:conclusion}.


% ============================================================

% THE CLEAN TEXT 
% agreeing on the wording:
% \begin{itemize}
%     \item {\bf remote sensing} is a technology
%     \item {\bf remote sensing imagery} is the class of visual data (certain measurements represented typically as raster/digital images acquired from satellites/aircraft/etc.
%     \item {\bf remote sensing images} is the class of visual data (certain measurements represented typically as raster/digital images acquired from satellites/aircraft/etc.
    
% \end{itemize}


% intro plan (claim - reason - evidence):
% \begin{enumerate}
%     \item deep learning approaches are even more expensive in terms of money spent on data, when things come to remote sensing applications 
%     \begin{enumerate}
%         \item reason 1: 
%     \end{enumerate}

%     \item why change detection is our example target application: representative/challenging in terms of getting high-quality labeling
%     \begin{enumerate}
%         \item reason 1: 
%     \end{enumerate}

%     \item software tools increasingly used for synthesis of realistic training data as many more tools are becoming freely available etc. 
%     \begin{enumerate}
%         \item reason 1: 
%     \end{enumerate}

% \end{enumerate}

% {\bf main finding \#1:} augmenting the training sets with synthetic data helps improve recognition rates in many ways 

% {\bf main finding \#2:} we have found how to create such a synthetic data using ``cheap'' procedural tools -> goes into MON grant report 




% ============================================================



% Remote sensing and aerial imagery services are widely used for many industrial and commercial projects. The recent years show a growing trend of commercialization of remote sensing projects ([1]).

% Remote sensing technology is a powerful tool for monitoring deforestation, wildfire, illegal construction and urban growth. These applications are fundamentally important for ecosystem management, security, business and analytics.


% As an example, detecting oil pipeline leaks over a series of remote sensing images has been topical since the 1990s, while tracking agricultural land use and forests cover changes via satellite imagery has been considered since the 1970s. 


% Analyzing time series of images is also relevant for such domains as medicine, robotics and others where the imagery represents the dynamics of objects or physical processes.


% Detecting structural changes in aerial images is a challenging problem, as illustrated in figure \ref{fig:challenge}. 

% \begingroup
% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=0.8\columnwidth]{figures/change_detection_in_out.png}
% \caption{Visualization of formal change detection task setting, where target change class is building emergence}
% \label{fig:challenge}
% \end{center}
% \end{figure}
% \endgroup

% Images taken at distinct dates may contain both structural changes (construction, building demolition, traffic signs) and nuisances such as viewpoint changes, outdoor conditions (lighting, weather, season) and dynamic changes (vehicles, vegetation). 

% Formally, the task of change detection, that is used in this work is the following:\\
% $I \in \{0, 1, ... , 255\}$ - an integer intensity of a pixel. \\
% $P \in I^3$ - a triplet of numbers representing RGB intensities of a pixel. \\
% $A_1, A_2 \in P^{m \times n}$— a pair of input images and $b \in I^{m \times n}$— a pixelwise binary mask.\\

% Given $A_1, A_2$ predict $b$,where 
% \begin{align}
%     b_{i,j} = 
% \begin{cases}
%      {255}, & \text{if pixel }(i,j) \text{ is in target change between }\\&
%      \text{pixels of }A_{1_{i,j}} \text{ and }A_{2_{i,j}}\\
%      0,& \text{otherwise}\\
%     \end{cases}
% \end{align}
% Traditional methods for detecting changes in image sequences include morphological analysis, multivariate regression analysis, multivariate alteration detection, uncontrolled classification and others. Currently, they can neither outperform deep learning approaches in terms of performance or robustness since they rely heavily on hand-crafted features or specific assumptions about data distribution (for instance, in the case of regression, based on Gaussian processes).
 
% Convolutional neural networks show great potential in remote-sensing applications due to their ability to undercover underlying features and structures of observational data. However, in order to successfully differentiate between structural changes and rеgular variations, the detection model requires large amount of high-quality annotated data. 

% Although labeling image segmentation datasets is highly resource-consuming there are several more issues concerning the problem of change detection in remote sensing imagery:
% \begin{enumerate}
% \item Change detection is an imbalanced class problem: some changes rarely occur naturally, so it might be a challenge to collect a representative number of positive examples. 
% \item Remote sensing and aerial data is expensive. Along with an imbalanced classes problem, dataset collection becomes highly expensive. 
% \item Manual markup is required, which is also a time- and resource-consuming procedure. 
% \end{enumerate}

% In various domains a common way to avoid regular dataset collection issues is to create a synthetic set of training data. Latest game development software powered by GPUs allow to simulate diverse physical conditions and generate realistic images. Pretrained on synthetic data, deep learning models can be used for training/fine-tuning on real data. 
% Works like \cite{}[45] show the success of synthetic data approach in the domain of object detection (see 1-2). 
% Overall, the potential benefits of using synthetic data generation pipeline are the following:
% \begin{enumerate}
% \item This approach implies flexibility in scene composition (including procedural objects placement and background variations)  which allows to solve imbalanced classes problems due to rich semantics.
% \item Procedural labeling is fully pixel precise and does not require manual markup.
% \end{enumerate}
% Despite these advantages, data syntheses with game engines has its own challenges:
% \begin{enumerate}
% \item Large-scale urban scenes consist of many objects, which require sufficient computational resources to keep them in memory simultaneously and handle procedural scene changes. 
% \item Even middle sized scenes require significant optimization either at the scene-level (rendering settings, shaders optimization, shadow casting etc.) or the object-level (reduction of polygons and textures quality).
% \item To get a realistic picture, one needs to either spend much time modeling and optimizing the scene or buy ready-made assets, which are expensive and unoptimized.
% \end{enumerate}
% Thus, the aim of this work is to investigate whether the approach of transfer learning from synthetic data applied to remote sensing and aerial imagery change detection will help to improve model performance.

% Therefore, we have stated the following goals of this work: 
% \begin{enumerate}
% \item To overview existing 3D procedural generation tools and implement a pipeline for synthetic dataset generation; 
% \item  To generate a synthetic change detection dataset;
% \item To evaluate model performance on the generated and real data. 
% \end{enumerate}

==> 03-methods.tex <==
\section{Synthesis of territory-specific remote sensing images}
\label{sec:methods}

\subsection{Data requirements and the design choices of our pipeline}
\label{methods:requirements_tools}


% \begingroup
% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=0.95\columnwidth]{compressed/geomtry-shading-rendering.jpg}
% \caption{Proposed pipeline for synthetic data generation}
% \label{fig:pipeline}
% \end{center}
% \end{figure}
% \endgroup

A good change detection dataset should contain application-specific target changes, such as, \eg, deforestation or illegal construction, as well as high variability, which can be viewed as non-target changes. Such variability in data commonly involves appearance changes, \eg, lighting and viewpoint variations, diverse directions of shadows, and random changes of scene objects; the more variability is embodied in the dataset, the more successful will be the transfer of experience from synthetic data to real ones. However, implementing an exhaustive list of non-target changes is difficult, as excessively many requirements for synthetic data make implementation too labourous. Thus, we restricted ourselves to the following \emph{general requirements} to the synthetic data:

\begin{itemize}  
    \item \textit{Visual scene similarity.} To reduce the omnipresent \emph{simulated to real} shift, it is necessary that the modelled scenes have high visual similarity to the real scenes. We approach the target territory modelling task by imitating the visual appearance of structures and environment. % We adjust buildings style/pick specific textures/colors

    \item \textit{Scale.} In order to match the largest known datasets in spatial scale, we have chosen to model scenes with large spatial size. 
    In our dataset, scenes are generated with spatial extents of square kilometers, spatial resolution of less than 1\,m, and image resolution of tens of Megapixels.
    % In our dataset, scenes are generated with spatial extents of approximately $2 \times 2$\,km$^2$ with spatial resolution of 0.6\,m and image resolution of $3072 \times 3072$\,pixels.
    
    \item \textit{Target changes.} We have chosen to only model damaged buildings as target class as they are of general interest in applications such as emergency mapping (see, \eg, \cite{jianya2008review,jabari2016building,tewkesbury2015critical,saha2018unsupervised,el2017zoom,wiratama2018dual,bai2018towards,el2016convolutional,vittek2014land,huang2015automatic}). They are also straightforward to implement in our pipeline with procedural geometry generation and rendering scripts.
    
    \item \textit{Viewpoint variations}. Real-world multi-temporal remote sensing images for the same territory are commonly acquired using varying devices (\eg, devices with different field of view) and viewpoints. The acquisition is commonly performed at angles not exceeding 25~deg., and the data are then post-processed by registration and geometric correction. In our pipeline, we imitate the precession of a real satellite by randomly changing the image acquisition angle and the field of view.
    
    \item \textit{Scene lighting changes}. Scene illumination is commonly considered to consist of an point-source illumination (produced by the Sun) and an ambient illumination due to the atmospheric scattering of the solar rays. In our work, we consider the changes in the Sun's declination angle and model both components of the illumination.
 
    \item \textit{Shadows}. Real-world objects cast shadows that are irrelevant variations, and should be ignored. We model realistic shadows again by varying the Sun's declination angle. 

\end{itemize}

\begingroup

\begin{figure}[t]
\begin{center}
% \fbox{\rule{0}{6em}\rule{0.8\columnwidth}{0}}
\includegraphics[width=0.8\columnwidth]{compressed/terrain_reconstruction_texturing.jpg}
\caption{Terrain reconstruction: (a) cartographic data, (b) altitude data, (c) model of reconstructed terrain.}
\label{fig:terrain_reconstruction_texturing}
% \end{center}
% \end{figure}
\bigskip
% \begin{figure}[!htb]
% \begin{center}
% \fbox{\rule{0}{6em}\rule{0.8\columnwidth}{0}}
\includegraphics[width=0.8\columnwidth]{compressed/extrusion_roofs_texturing.jpg}
\caption{Geometry generation: (a) polygon extrusion, (b) adding roofs, (c) texturing.}
\label{fig:extrusion_roofs_texturing}
\end{center}
\end{figure}

\endgroup

To meet these requirements we have developed a~two-stage pipeline consisting of geometry generation and rendering steps. The entire routine is semi-automatic and involves two widely used 3D engines. Specifically, we use \emph{Esri CityEngine}~\cite{cityengine} to proceduraly build geometry from real-world map data and~\emph{Unity}~\cite{unity3d} to implement the logic behind dataset requirements and leverage rendering capabilities. The reasons behind our choice of \emph{CityEngine} as our geometry manipulation tool are its flexibility in the procedural geometric modelling and built-in UV/texturing capabilities. Other tools, commonly implemented as plugins for \emph{Unreal Engine 4} (\eg, \emph{StreetMap}\footnote{\url{https://github.com/ue4plugins/StreetMap}}) and \emph{Unity} (\eg, \emph{Mapbox Unity SDK}\footnote{\url{https://www.mapbox.com/unity}}), offered significantly less freedom. In these tools, either non-textured or textured but oversimplified shapes (\eg, as simple as boxes) are the only objects available for urban geometry generation.

\emph{Unity} game engine was selected to execute a generation procedure of change detection dataset. Compared to CAD software often used for the production of datasets, game engines offer advantages such as powerful lighting out of the box, realistic computation of shadows, and scripting possibilities. Additionally, \emph{Unity} allows implementing target changes, controlling lightning and viewpoint changes, and adjusting change rate in the dataset. Certain features in \emph{Unity} are more suited to our needs, compared to \emph{Unreal Engine 4}. For instance, we have found shadows in \emph{Unity} to be more stable while rendering scenes from large distances, and the \emph{Layers} feature\footnote{\url{https://docs.unity3d.com/Manual/Layers.html}} to add more flexibility by allowing to exclude objects from rendering or post-processing. It is natural, however, that we had to execute some initial settings of \emph{Unity} before the generation, as the typical requirements of the remote sensing domain differs from those of 3D games. We describe these settings in Section~\ref{sec:experiments}. 

% \LA{decide what to do with the paragraph}
% We use CityEngine to extrude geometry from polygons obtained via OpenStreetMap. The building textures are applied there as well. The terrain shading procedure is based on Unity3d shader script that leverages rasterized vector layers from OpenStreetMap. 

% An overview of our generation pipeline is presented in Figure~\ref{fig:pipeline}. We further describe every step in greater detail.



\subsection{Geometry generation}
\label{methods:geometry}

To procedurally generate geometry in \emph{CityEngine}, we obtain cartographic data (vector layers) from \emph{OpenStreetMap} and elevation data (a~geo-referenced GeoTIFF image) from \emph{Esri World Elevation}. Vector data contains information about the geometry of buildings and roads along with semantics of land cover (forests, parks, \etc), while elevation data is used to reconstruct terrain.

First, we reconstruct terrain using the built-in functionality in \emph{CityEngine}, obtaining a textured 3D terrain mesh (see Figure~\ref{fig:terrain_reconstruction_texturing}), to which we $z$-align flat vector objects; second, we run our geometry generation procedure implemented in the engine's rule-based scripting language; last, we apply textures to the generated meshes. Our implementation of the geometry generation involves extruding the polygon of a certain height and selecting a randomly textured roof (architectural patterns such as rooftop shapes are built into \emph{CityEngine}), see Figure~\ref{fig:extrusion_roofs_texturing}. We have experimented more complex geometry produced by operations such as polygon splitting and repeating, however, some such operations (\eg, splitting) increase the number of polygons significantly without adding much to the scene detail, render quality, or performance of change detection models. Focusing on our scalability and flexibility requirements, we avoid overloading our scenes with objects of redundant geometry. % to keep our tool highly flexible. %, while being prohibitively costly when working with large scenes. 


We select two types of buildings to construct our scenes: small buildings with colored gable roofs and concrete industrial-looking structures with flat roofs, see Figure~\ref{fig:buildings_realism}. A set of roof textures has been selected manually, \emph{CityEngine} built-in packs of textures for \emph{OpenStreetMap} buildings were used for facades.

We approach the emergency mapping use-case by texturing buildings footprints to imitate damaged appearance. A simple rule was implemented to address this issue: the building polygon is slightly scaled up, a texture with transparency is applied further, see Figure~\ref{fig:structures_ashes}.



\begingroup

\begin{figure} %[htbp]
\begin{minipage}[t]{0.49\linewidth}
    \begin{center}
    % \fbox{\rule{0}{6em}\rule{1.0\columnwidth}{0}}
    \includegraphics[width=1.0\columnwidth]{compressed/structures_ashes.jpg}
    \caption{Addressing the case of emergency mapping: scene model (a) before and (b) after the emergency situation (note that some structures are missing).}
    \label{fig:structures_ashes}
    \end{center}
\end{minipage}%
    \hfill%
\begin{minipage}[t]{0.45\linewidth}
    \begin{center}
    % \fbox{\rule{0}{6em}\rule{0.8\columnwidth}{0}}
    \includegraphics[width=1.0\columnwidth]{compressed/buildings_realism.jpg}
    \caption{The two models of buildings used in our pipeline: (a) photo and (c) our render of \emph{residential houses}, (b) photo and (d) our render of \emph{industrial structures}.}
    \label{fig:buildings_realism}
    \end{center}
\end{minipage} 
\end{figure}

\endgroup



% \subsection{Shading}
% \label{methods:shading}

% The motivation behind this stage is to mask the flaws of low-resolution satellite images, that might not be aligned with geometry, yielding false shadows or flat objects in renders. We implement shaders in \emph{Unity} with a specific OpenGL-like language. The simplest definition of our terrain shading routine is to fill regions corresponding to a set of classes (\eg, forest, field, roads, ground) with corresponding textures. The surface localization is obtained via \emph{OpenStreetMap} vector layers. The details are extracted from corresponding satellite imagery. The next step is to collect the texture samples for each class. Along with flat surface texturing some vegetation spanning logic has been implemented too. A specific point can be chosen in the scene to place a spawning object. One needs to define the radius, density and the set of tree models to be picked from randomly.



\subsection{Rendering}
\label{methods:rendering}

% 1. Why we do rendering: this is a way to 
% - generate images
% - add diversity to dataset
% 2. How we do rendering: Unity pipeline + reference to specifications
% - Unity features we use (built-in algorithms, picking changes, we specify the most optimal, subject to our experience)
% - how we obtain annotations 

We construct the synthetic dataset by rendering the generated geometry using built-in functionality in \emph{Unity}, obtaining high-definition RGB images. When producing these images, our goal is to introduce the diversity to the data by adding both target changes (\eg, damaged buildings) and non-target variations (lighting and viewpoint changes). 

To achieve a high degree of variations, we leverage rich scripting capabilities in \emph{Unity}, that allow flexible scene manipulation via scripts written in C\#. As shadow casting and lighting algorithms are built in, we only adjust their parameters, as indicated in Section~\ref{experiments:datasets}. We implement target changes by randomly selecting object meshes and placing them onto the separate layer: the camera will not render these meshes, rendering corresponding damaged footprints instead. Non-target variations are further added to scenes modified by target changes, by random alterations of lighting and camera parameters, resulting in $m$ different image acquisition conditions per each target change. 

Each element in the dataset was obtained after three rendering runs: first, we render the original scene; second, we apply both target and non-target changes, moving the changed objects in the separate layer; finally, only the layer with the changed objects is rendered to obtain annotations.


% % move to experiments section
% For each scene setup ten images are generated (5 pre-event/5 post-event). To make a dataset element a random image is picked over 5 for each time period, thus getting a pair of images ``before'' - ``after'', shot from different viewpoints. A corresponding ground truth mask is picked from either sample - the displacement due to the viewpoint difference is handled during orthographic correction. 

% The following section draws the procedure in details.


